Hypercontracts

Contract theories have been proposed to formally support distributed and decentralized system design while ensuring safe system integration. In this paper we propose hypercontracts, a generic model with a richer structure for its underlying model of components, subsuming simulation preorders. While this new model remains generic, it provides a much more elegant and richer algebra for its key notions of refinement, parallel composition, and quotient, and it allows inclusion of new operations. On top of these foundations, we propose conic hypercontracts, which are still generic but come with a finite description.

==> appendices/additionalReceptiveProofs.tex <==

%\begin{proof}[Proof of Proposition \ref{hbaixoib}]
    \begin{proof}[Proof of Proposition 5.7]
    
\end{proof}

==> appendices/hypercontractsAndAgContracts.tex <==


Now we express AG contracts using hypercontracts. 
We can
instantiate trace properties as a $\catCmpSet$ lattice. Each \compset is of the
form $\cmpSet = 2^\cmp$ for some component $\cmp \subseteq \behaviorUnv$.
Observe that the satisfaction of a \compset by a component $\cmp' \in 2^{\cmp}$
happens if and only if $\cmp' \le \cmp$. The meet of two \compsets $2^\cmp \meet
2^{\cmp'}$ is $2^{\cmp \setint \cmp'} = 2^{\cmp} \setint 2^{\cmp'}$, but the
join of two elements $2^\cmp \vee 2^{\cmp'}$ is $2^{\cmp \setunion \cmp'} \ne
2^\cmp \setunion 2^{\cmp'}$. The composition of two \compsets is given by
$2^{\cmp} \times 2^{\cmp'} = 2^{\cmp \setint \cmp'}$, and the quotient is
$2^{\cmp} / 2^{\cmp'} = 2^{\cmp / \cmp'}$.

Assume-guarantee contracts are often given as a
pair of trace-properties $(A, G)$, where $A$ states the assumptions made on the
environment, and $G$ states what the component in question should guarantee when
operating in a valid environment (i.e., one that meets the assumptions). We
observe that any closed system obtained using environments that meet the
assumptions is restricted to $G \setint A$; thus, we set the closed-system spec
to $\sysSet = 2^{A \setint G}$. Define the hypercontract $\cont = (2^A, 2^{A
\setint G})$. The environments are $\envSet = 2^A$, namely, all $E \subseteq A$,
and the implementations are $\impSet = 2^{(A \setint G)/A} = 2^{G / A}$, that
is, all $\cmp \subseteq G / A$. Observe that $\sysSet / \impSet = \envSet$, so
$\cont$ is saturated. Now suppose we have another hypercontract $\cont' =
(2^{A'}, 2^{A' \setint G'})$ with environments $\envSet'$ and implementations
$\impSet'$. We observe that $\envSet \le \envSet'$ if and only if $A \subseteq
A'$; moreover, $\impSet' \le \impSet$ if and only if $G' / A' \le G / A$. This
means that $\cont' \le \cont$ if and only if the assume-guarantee contracts $(A,
G)$ and $(A', G')$ satisfy $(A', G') \le (A, G)$.

Suppose we
have a second hypercontract $\cont' = (2^{A'}, 2^{G' / A'})$. Applying
\eqref{eq:cntComp}, we obtain a composition formula for these hypercontracts:
$\cont \contComposition \cont' = \left( 2^{A' / (G / A)} \right. \meet \linebreak[1] \left. 2^{A/(G'/A')},
2^{G/A} \meet 2^{G'/A'} \right)$, whose environments and implementations are
exactly those obtained from the composition of the assume-guarantee contracts
$(A, G)$ and $(A', G')$ \cite{Benveniste2008}.

Given two assume-guarantee contracts $(A_i, G_i)$
for $i = 1,2$, we consider the merging of their hypercontracts. We have
$(2^{A_1}, 2^{A_1 \setint G_1}) \bullet (2^{A_2}, 2^{A_2 \setint G_2}) = (2^{A_1
\setint A_2}, 2^{A_1 \setint G_1 \setint A_2 \setint G_2})$. Observe that this
last hypercontract has environments $2^{A_1 \setint A_2}$ and implementations
$2^{(G_1 \setint G_2) / (A_1 \setint A_2)}$. This is the definition of merging
for assume-guarantee contracts \cite{agContractMerging}.

%Appendix \ref{xknskaJK} shows a novel extension of AG contracts in which
%environments and implementations are allowed to state not only allowed
%behaviors, but also required behaviors, in the style of modal interfaces.


==> sections/applications.tex <==




\begin{comment}
\subsection{Application: Robustness of 
%data-driven 
Machine Learning systems}

In recent years, systems developed for an increasing number of verticals
comprise
%data-driven 
Machine Learning (ML) components. This has spurred an interest in proving
properties about these components, particularly since some of these systems are
used in safety-critical applications. Yet, even stating what to prove comes with
challenges, as ML methodologies are employed when we lack in advance a
known mathematical relation between an input and an output space, whereas the
statement of a formal property usually requires us to state the behavior that we
wish the system to have.

It has been shown
that existing ML components can be brittle, in the sense that small changes to
inputs can produce large changes in their outputs 
\cite{szegedy2014intriguing}. 
Thus, we are often interested in
showing that ML systems are robust: if the inputs to the ML component are
sufficiently close, the outputs should be sufficiently close
\cite{formalSpecsDnns}. Suppose $\inSpace$ and $\outSpace$ are the input and
output spaces where the ML component operates. In a supervised setting, we start
with a finite set of samples $\{(x_i, y_i)\}_{i=1}^N$, where $x_i \in \inSpace$
and $y_i \in \outSpace$ for all $i$. Using this set, a learning algorithm
generates a function $f: \inSpace \to \outSpace$. If $d_\inSpace$ and
$d_\outSpace$ are distance metrics on the input and output spaces, for a given
$x \in \inSpace$, we can ask that the function be robust against small
variations around $x$ through the hyperproperty $\forall x' \in \inSpace.\,\,
d_\inSpace(x,x') < \delta \Rightarrow d_\outSpace(f(x), f(x')) < \varepsilon$
for some nonzero $\delta$ and $\epsilon$.
%
In the case of a classification task, where $\outSpace$ is finite,
%we may wish to state that inputs belonging to certain regions of the input space are mapped to given labels. Doing this suggests that we have a mathematical description of how the classification should be effected (which may render learning unnecessary). The goal with stating these properties is considerably more modest: 
we can state that inputs which are close in some metric to the samples
corresponding to a known class are mapped to that class.
%Note that if we
%enforced this property on the entire input space, and assuming that this
%space is connected, the entire input space would map to the same label. Thus, it
%is important that we check for robustness against input variations around a set
%of inputs known to belong to certain classes.

\newcommand{\stopSpace}[0]{\mathcal{S}}
\newcommand{\classifierSpace}[0]{\mathcal{F}}

Consider a vehicle approaching an intersection with a stop sign. We wish
the vehicle to respect the hypercontract $\cont = $ (all driving conditions, if
there is a stop sign then stop vehicle within a distance $D$ from the stop
sign). The implementations say that the vehicle must do something when an object
is present in the physical world. An ideal perception hypercontract would be
something like $\cont_p = $ (all driving conditions, say there is a stop sign if
and only if there is a stop sign in the real world). Now we can let $\inSpace$
be the space of all possible images one can encounter while driving. Then we can
say that $\stopSpace \subseteq \inSpace$ is the subset of images containing a
stop sign. Currently we have no means for characterizing $\stopSpace$, but we
construct, for example, an approximation $\hat \stopSpace$ containing all images
which are close in some metric to images known to have stop signs. Suppose we
partition the input space in $n+1$ regions $\hat S$, $\inSpace_1, \ldots,
\inSpace_n$, where $\inSpace_i$ is smaller than a $d_\inSpace$-ball of radius
$\delta$. If we train a classifier $f$ to recognize $K$ different categories, we
require this classifier to map the values belonging to a set in the partition to
one specific class. Since the values of $\hat \stopSpace$ must map to the stop
sign, the only choice is for the rest of the elements of the partition. This
means that there are $K^n$ possible classifiers. Call $\classifierSpace$ the set
of all $K^n$ possible classifiers. If we call $x$ the image input provided by
the environment and $y$ its assigned class, the perception hypercontract can
become
\[
    \cont_p = (\langle \text{all possible images} \rangle,  \left\langle y =  f(x) \right\rangle_{f \in \classifierSpace}).
\]
This hypercontract has a 1-\maximal environment set and a $K^n$-\maximal
implementation set.
However, the perception hypercontract, likely implemented by a neural network, is still
too removed from the description of the high-level hypercontract $\cont$. We can
bridge the gap by writing the high-level hypercontract as
\[
    \cont = (\langle x \in \inSpace \rangle,  x \in \hat \stopSpace \Rightarrow  \text{stop vehicle within a distance $D$ from the stop sign} ).
\]

Now both the system spec and the perception spec are given at the same level of
abstraction. Thus, using the quotient we can focus on what the perception
specification does not capture, namely, the control aspects of the design.

\end{comment}
\begin{comment}
\subsection{Continuous systems}

We use hypercontracts to consider an application of
 assume-guarantee reasoning to continuous systems as carried out by
 \cite{DBLP:conf/eucc/SaoudGF18,saoud:hal-02196511}. Suppose we have a finite
 set $\alphabet$ of connected subsets of $\mathbb{R}$. We will think of an
 element of $\alphabet$ as a ``continuous variable.'' These variables fulfill
 the roles of inputs and outputs for continuous systems; we think of state as an
 additional output to simplify our notation. For a given nonnegative real number
 $T$, the set $\behaviorUnv$ of behaviors consists of all functions of the form
 $[0,T] \to \prod_{X \in \alphabet} X$.

We call an IO signature of $\alphabet$ a partition of $\alphabet$ into two sets
$(I,O)$ of input and output variables. The set of \emph{components with input
$I$}, denoted $\cmpUniverse_I$, consists of all subsets $M \subseteq
\behaviorUnv$ such that if $f \in M \land \text{Dom}(f) = [0, T]$ then
$f_{[0,T']} \in M$ for all $0 \le T' \le T$. This means that components contain
all time prefixes of the behaviors they can display. Observe that we interpret
$M$ as having inputs $I$ and outputs $O$. The set of components of the theory is
$\cmpUniverse = \oplus_{I \in 2^{\alphabet}} \behaviorUnv_I$.

The composition of two components $M$ and $M'$ with IO signatures $(I, O)$ and
$(I',O')$, respectively, is defined when the components share no outputs, i.e.,
when $I \setunion I' = \alphabet$. In that case, the composite $\behaviorUnv_I
\contComposition \behaviorUnv_{I'} \to \behaviorUnv_{I \setint I'}$ is $M
\setint M'$. Observe that the composite has outputs $O \setunion O'$ and inputs
$I \setint I'$.

If we define $\catCmpSet$ as the lattice consisting of all 1-\conic sets
($2^M$), we can express properties like invariance (the system variables belong
to some set at all times) and differential inclusion (the vector of time
derivatives of a behavior belongs to a time-invariant set). Saoud et al.
\cite{saoud:hal-02196511} show that if there are components $\{M_i\}_{i = 1}^n$
and hypercontracts $\{\cont_i = \left(2^{A_i}, 2^{G_i}\right)\}_{i = 1}^n$ such
that $M_i \satImpl \cont_i$, the acyclic composition of this objects satisfies
the hypercontract $\cont = \left(\setint_i 2^{A_i}, \setint_i 2^{G_i}\right)$.
They also show that under stricter conditions on the components, one can obtain
the same result for arbitrary connection topologies.


\end{comment}


